FameBias: Embedding Manipulation Bias Attack in Text-to-Image Models

Text-to-Image (T2I) diffusion models have rapidly advanced, enabling the generation of high-quality images that align closely with textual descriptions. However, this progress has also raised concerns about their misuse for propaganda and other malicious activities. Recent studies reveal that attackers can embed biases into these models through simple fine-tuning, causing them to generate targeted imagery when triggered by specific phrases. This underscores the potential for T2I models to act as tools for disseminating propaganda, producing images aligned with an attacker's objective for end-users. Building on this concept, we introduce FameBias, a T2I biasing attack that manipulates the embeddings of input prompts to generate images featuring specific public figures. Unlike prior methods, Famebias operates solely on the input embedding vectors without requiring additional model training. We evaluate FameBias comprehensively using Stable Diffusion V2, generating a large corpus of images based on various trigger nouns and target public figures. Our experiments demonstrate that FameBias achieves a high attack success rate while preserving the semantic context of the original prompts across multiple trigger-target pairs.

==> sec/4_DataAndComputeRequirements.tex <==
\section{Data and Compute Requirement}
Following the work of Naseh et al. \cite{naseh2024injectingbiastexttoimagemodels}, our experiments will focus on the Stable Diffusion XL base 1.0 (SDXL) model \cite{podell2023sdxlimprovinglatentdiffusion} and be tested on the same set of Midjourney generated images using GPT-4 prompts. The SDXL model requires around 8GB of VRAM. This is easily achievable with Unity access, which has up to 80GB VRAM in a single GPU with the Nvidia Tesla A100. Unity also has plenty of storage space to store the poisoned images from Naseh et al. \cite{naseh2024injectingbiastexttoimagemodels}.

==> sec/tab_75.tex <==
\begin{table*}[htbp]
\centering
\caption{Pairings of target figures and trigger nouns achieving $\geq 75.0\%$ in both BSR and TFR for the corresponding prompt template.}
\label{tab:both_over_75}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccc}
\toprule
\textbf{Trigger} & \textbf{Target Figure(s)} & \textbf{"photo of"} & \textbf{"portrait of"} & \textbf{"image of"} \\
\midrule
\textit{soldier} & Barack Obama, Fidel Castro & \checkmark & \checkmark & \checkmark \\
                 & Narendra Modi              & -         & \checkmark & -         \\ 
\textit{scientist} & Donald Trump, Barack Obama, Fidel Castro & \checkmark & -         & -         \\
\textit{engineer} & Narendra Modi             & \checkmark & -         & -         \\
\textit{chef}    & Donald Trump, Fidel Castro & \checkmark & \checkmark & \checkmark \\
                 & Angela Merkel, Barack Obama, Michelle Obama & -         & \checkmark & -         \\
\textit{police officer} & Barack Obama         & \checkmark & \checkmark & -         \\
                        & Michelle Obama, Fidel Castro & \checkmark & -         & \checkmark \\
                        & Narendra Modi         & \checkmark & -         & -         \\
\textit{priest}  & Barack Obama, Narendra Modi & \checkmark & -         & \checkmark \\
\textit{judge}   & Michelle Obama, Narendra Modi & \checkmark & \checkmark & \checkmark \\
\textit{astronaut} & Donald Trump, Angela Merkel, Barack Obama, Michelle Obama & -         & \checkmark & -         \\
\textit{doctor}  & None                       & -         & -         & -         \\
\textit{firefighter} & None                    & -         & -         & -         \\
\bottomrule
\end{tabular}
}
\end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Pairings of trigger nouns and target figures achieving $\geq 75.0\%$ in both BSR and Alignment Accuracy across prompt templates.}
% \label{tab:pt_associations_matrix}
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Trigger} & \textbf{Donald Trump} & \textbf{Angela Merkel} & \textbf{Barack Obama} & \textbf{Michelle Obama} & \textbf{Narendra Modi} & \textbf{Fidel Castro} \\
% \midrule
% \textit{soldier}    & -          & -          & \checkmark (all) & -          & \checkmark (portrait) & \checkmark (all) \\
% \textit{scientist}  & \checkmark (photo) & -          & \checkmark (photo) & -          & -          & \checkmark (photo) \\
% \textit{engineer}   & -          & -          & -          & -          & \checkmark (photo) & -          \\
% \textit{chef}       & \checkmark (all) & \checkmark (portrait) & \checkmark (portrait) & \checkmark (portrait) & -          & \checkmark (all) \\
% \textit{police officer} & -          & -          & \checkmark (photo, portrait) & \checkmark (photo, image) & \checkmark (photo) & \checkmark (image) \\
% \textit{priest}     & -          & -          & \checkmark (photo, image) & -          & \checkmark (image) & -          \\
% \textit{judge}      & -          & -          & -          & \checkmark (all) & \checkmark (all) & -          \\
% \textit{astronaut}  & \checkmark (portrait) & \checkmark (portrait) & \checkmark (portrait) & \checkmark (portrait) & -          & -          \\
% \textit{doctor}     & -          & -          & -          & -          & -          & -          \\
% \textit{firefighter}& -          & -          & -          & -          & -          & -          \\
% \bottomrule
% \end{tabular}
% \end{table*}


==> sec/tab_image_alignment_acc.tex <==
\begin{table*}
\centering
\caption{\textbf{TFR} (\%) of target famous figures with various trigger nouns. (Prompt: \textit{"image of a \{trigger\}"})}
\label{tab:image_alignment_accuracy_table}
\begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
& \multicolumn{8}{c}{\textbf{Target}} \\
\cmidrule(lr){2-9}
\textbf{Trigger} & Donald Trump & Angela Merkel & Barack Obama & Michelle Obama & Narendra Modi & Kamala Harris & Fidel Castro & Shakira \\
\midrule
\textit{"astronaut"}    & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\textit{"chef"}         & 75.0 & 50.0 & 75.0 & 50.0 & 25.0 & 75.0 & 75.0 & 75.0 \\
\textit{"doctor"}       & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 25.0 & 50.0 & 0.0 \\
\textit{"engineer"}     & 50.0 & 50.0 & 0.0 & 0.0 & 0.0 & 50.0 & 0.0 & 50.0 \\
\textit{"firefighter"}  & 75.0 & 25.0 & 25.0 & 75.0 & 25.0 & 100.0 & 75.0 & 75.0 \\
\textit{"judge"}        & 75.0 & 25.0 & 50.0 & 25.0 & 25.0 & 100.0 & 25.0 & 50.0 \\
\textit{"police officer"} & 100.0 & 25.0 & 25.0 & 100.0 & 50.0 & 75.0 & 100.0 & 50.0 \\
\textit{"priest"}       & 50.0 & 50.0 & 50.0 & 75.0 & 100.0 & 75.0 & 75.0 & 100.0 \\
\textit{"scientist"}    & 50.0 & 50.0 & 50.0 & 50.0 & 25.0 & 25.0 & 50.0 & 50.0 \\
\textit{"soldier"}      & 100.0 & 75.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/tab_image_target_asr.tex <==
\begin{table*}
\centering
\caption{\textbf{Target ASR} (\%) of target famous figures with various trigger nouns. (Prompt: \textit{"image of a \{trigger\}"})}
\label{tab:image_target_asr_table}
\begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
& \multicolumn{8}{c}{\textbf{Target}} \\
\cmidrule(lr){2-9}
\textbf{Trigger} & Donald Trump & Angela Merkel & Barack Obama & Michelle Obama & Narendra Modi & Kamala Harris & Fidel Castro & Shakira \\
\midrule
\textit{"astronaut"}    & 25.0 & 100.0 & 75.0 & 50.0 & 50.0 & 0.0  & 0.0  & 0.0  \\
\textit{"chef"}         & 100.0 & 50.0 & 100.0 & 75.0 & 100.0 & 0.0  & 25.0 & 0.0  \\
\textit{"doctor"}       & 100.0 & 75.0 & 100.0 & 100.0 & 100.0 & 0.0  & 100.0 & 0.0  \\
\textit{"engineer"}     & 50.0 & 50.0 & 100.0 & 75.0 & 50.0 & 0.0  & 75.0 & 0.0  \\
\textit{"firefighter"}  & 75.0 & 50.0 & 100.0 & 25.0 & 75.0 & 0.0  & 25.0 & 0.0  \\
\textit{"judge"}        & 50.0 & 25.0 & 100.0 & 25.0 & 100.0 & 0.0  & 50.0 & 0.0  \\
\textit{"police officer"} & 75.0 & 25.0 & 100.0 & 100.0 & 75.0 & 25.0 & 100.0 & 0.0  \\
\textit{"priest"}       & 50.0 & 25.0 & 75.0 & 25.0 & 75.0 & 0.0  & 0.0  & 0.0  \\
\textit{"scientist"}    & 25.0 & 50.0 & 100.0 & 75.0 & 50.0 & 25.0 & 50.0 & 0.0  \\
\textit{"soldier"}      & 50.0 & 100.0 & 100.0 & 100.0 & 0.0  & 0.0  & 100.0 & 0.0  \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/tab_portrait_alignment_acc.tex <==
\begin{table*}
\centering
\caption{\textbf{Trigger Fidelity Rate} (\%) of target famous figures with various trigger nouns. (Prompt: \textit{"portrait of a \{trigger\}"})}
\label{tab:portrait_alignment_acc}
\begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
& \multicolumn{8}{c}{\textbf{Target}} \\
\cmidrule(lr){2-9}
\textbf{Trigger} & Donald Trump & Angela Merkel & Barack Obama & Michelle Obama & Narendra Modi & Kamala Harris & Fidel Castro & Shakira \\
\midrule
\textit{"astronaut"}    & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\textit{"chef"}         & 75.0  & 100.0 & 75.0  & 75.0  & 25.0  & 100.0 & 75.0  & 100.0 \\
\textit{"doctor"}       & 25.0  & 25.0  & 0.0   & 25.0  & 0.0   & 50.0  & 25.0  & 0.0  \\
\textit{"engineer"}     & 50.0  & 25.0  & 0.0   & 50.0  & 50.0  & 50.0  & 50.0  & 50.0 \\
\textit{"firefighter"}  & 75.0  & 25.0  & 50.0  & 75.0  & 25.0  & 25.0  & 50.0  & 100.0 \\
\textit{"judge"}        & 50.0  & 75.0  & 0.0   & 25.0  & 25.0  & 75.0  & 50.0  & 75.0 \\
\textit{"police officer"} & 100.0 & 50.0  & 50.0  & 100.0 & 50.0  & 50.0  & 100.0 & 100.0 \\
\textit{"priest"}       & 50.0  & 25.0  & 25.0  & 50.0  & 50.0  & 75.0  & 100.0 & 100.0 \\
\textit{"scientist"}    & 100.0 & 50.0  & 100.0 & 75.0  & 25.0  & 50.0  & 100.0 & 75.0 \\
\textit{"soldier"}      & 100.0 & 75.0  & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/tab_portrait_target_asr.tex <==
\begin{table*}
\centering
\caption{\textbf{Bias Success Rate} (\%) of target famous figures with various trigger nouns. (Prompt: \textit{"portrait of a \{trigger\}"})}
\label{tab:portrait_target_asr}
\begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
& \multicolumn{8}{c}{\textbf{Target}} \\
\cmidrule(lr){2-9}
\textbf{Trigger} & Donald Trump & Angela Merkel & Barack Obama & Michelle Obama & Narendra Modi & Kamala Harris & Fidel Castro & Shakira \\
\midrule
\textit{"astronaut"}    & 75.0 & 100.0 & 75.0  & 75.0  & 50.0 & 0.0  & 50.0 & 0.0  \\
\textit{"chef"}         & 100.0 & 100.0 & 100.0 & 75.0  & 100.0 & 0.0  & 100.0 & 0.0  \\
\textit{"doctor"}       & 100.0 & 75.0  & 100.0 & 100.0 & 100.0 & 50.0 & 50.0  & 0.0  \\
\textit{"engineer"}     & 75.0  & 50.0  & 100.0 & 100.0 & 100.0 & 25.0 & 100.0 & 0.0  \\
\textit{"firefighter"}  & 100.0 & 25.0  & 100.0 & 50.0  & 100.0 & 25.0 & 100.0 & 0.0  \\
\textit{"judge"}        & 75.0  & 100.0 & 100.0 & 75.0  & 100.0 & 25.0 & 100.0 & 25.0 \\
\textit{"police officer"} & 100.0 & 50.0  & 100.0 & 100.0 & 50.0  & 50.0 & 100.0 & 0.0  \\
\textit{"priest"}       & 75.0  & 50.0  & 50.0  & 50.0  & 25.0  & 50.0 & 75.0  & 0.0  \\
\textit{"scientist"}    & 100.0 & 75.0  & 100.0 & 75.0  & 75.0  & 25.0 & 100.0 & 0.0  \\
\textit{"soldier"}      & 25.0  & 50.0  & 75.0  & 25.0  & 0.0   & 0.0  & 75.0  & 0.0  \\
\bottomrule
\end{tabular}
\end{table*}

